Cascade RCNN for MIDOG Challenge

Mitotic counts are one of the key indicators of breast cancer prognosis. However, accurate mitotic cell counting is still a difficult problem and is labourious. Automated methods have been proposed for this task, but are usually dependent on the training images and show poor performance on unseen domains. In this work, we present a multi-stage mitosis detection method based on a Cascade RCNN developed to be sequentially more selective against false positives. On the preliminary test set, the algorithm scores an F1-score of 0.7492.

==> figures/retinanet.tex <==
\adjustbox{max width=0.5\textwidth}{
\begin{tikzpicture}[] 
\tikzstyle{every node}=[trapezium, draw, minimum width=3cm,
trapezium left angle=60, trapezium right angle=120]

% Encoder
\node[draw=none,
           path picture={
               \node at (path picture bounding box.center){
                   \includegraphics[width=4cm]{figures/mf.png}
               };
           }] at (0,-0.75) {};
\node[purple, minimum width = 3cm, fill=white, line width=1.5] (enc0) at (0,0) {};
\node[draw=none, purple, below = 1 cm of enc0, align=center] {ResNet Encoder}; 
\node[purple, minimum width = 2.5cm, fill=white, line width=1.5] (enc1) at (0,0.75) {};
\node[purple, minimum width = 2cm, fill=white, line width=1.5] (enc2) at (0,1.5) {};

% Decoder
\node[teal, minimum width = 3 cm, fill=white, line width=1.5, align = center] (dec0) at (5,0) {};
\node[draw=none, teal, below = 1 cm of dec0, align=center] {Feature Pyramid \\ Network}; 
\draw[->] (5,0.75) -- ($(dec0.center)+ (0,-0.2)$);
\node[teal, minimum width = 2.5cm, fill=white, line width=1.5] (dec1) at (5,0.75) {};
\draw[->] (5,1.5) -- ($(dec1.center)+ (0,-0.2)$);
\node[teal, minimum width = 2cm, fill=white, line width=1.5] (dec2) at (5,1.5) {};

\node[draw=none, align=center] (pred) at (9,0) {class + box \\ subnets};
\draw[->] (dec0.east) -- (pred.west);
\node[draw=none, align=center] (dis) at (0,3) {domain \\ discriminator};


\draw[->] ($(enc0.center)+ (0,-0.2)$) -| (enc1.south);
\draw[->] ($(enc1.center)+ (0,-0.2)$) -| (enc2.south);

\draw[->] (enc0.east) -- (dec0.center);
\draw[->] (enc1.east) -- (dec1.center);
\draw[->] (enc2.east) -- (dec2.center);
\draw[->, rounded corners] (enc2.center)  -- (dis.south);
\end{tikzpicture}}


